Federated Multimodal Learning with Dual Adapters and Selective Pruning for Communication and Computational Efficiency

Federated Learning (FL) enables collaborative learning across distributed clients while preserving data privacy. However, FL faces significant challenges when dealing with heterogeneous data distributions, which can lead to suboptimal global models that fail to generalize across diverse clients. In this work, we propose a novel framework designed to tackle these challenges by introducing a dual-adapter approach. The method utilizes a larger local adapter for client-specific personalization and a smaller global adapter to facilitate efficient knowledge sharing across clients. Additionally, we incorporate a pruning mechanism to reduce communication overhead by selectively removing less impactful parameters from the local adapter. Through extensive experiments on a range of vision and language tasks, our method demonstrates superior performance compared to existing approaches. It achieves higher test accuracy, lower performance variance among clients, and improved worst-case performance, all while significantly reducing communication and computation costs. Overall, the proposed method addresses the critical trade-off between model personalization and generalization, offering a scalable solution for real-world FL applications.

==> content/fig_tex/f_ablation.tex <==

\begin{figure}[]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{content/fig/a100_dir_ablationt_2_16_all_pfl.pdf}
        \caption{Apply LoRA on Text Encoder.}
        \label{fig:ablation_sora_t}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{content/fig/a100_dir_ablationv_2_16_all_pfl.pdf}
        \caption{Apply LoRA on Image Encoder.}
        \label{fig:ablation_sora_v}
    \end{subfigure}
    \caption{Comparison of performance with and without SoRA on the Aircraft dataset, showing accuracy and convergence improvements.}
    \label{fig:ablation_sora_combined}
\end{figure}



% \vspace{-2.0em}

% \label{fig:ablation}
% \end{center}
% \end{figure}

==> content/fig_tex/f_block.tex <==
\begin{figure}[ht]
% \vskip 0.2in
\begin{center}

% \vspace{-2.0em}

\centerline{\includegraphics[width=0.4\textwidth]{content/fig/block.pdf}}

\caption{The structure of each layer within the CLIP text encoder. Transformer blocks can be divided into two minimal residual blocks that can be analyzed independently~\cite{zhong2024blockpruner}.}

\vspace{-2.0em}

\label{fig:block}
\end{center}
\end{figure}

==> content/fig_tex/f_method.tex <==
\begin{figure*}[ht]
% \vskip 0.2in
\begin{center}

\centerline{\includegraphics[width=0.7\textwidth]{content/fig/overview.pdf}}

\caption{Different methods for local model update. The clients download the transferred model from the server, train locally with the local data, and upload it to the server. \textbf{\proj}: only transfer LoRA Adapter; \textbf{FedAA}: only transfer Attention Adapter; \textbf{FedLC}: only transfer Linear Classfier; \textbf{FedVM-LC}: only transfer Vision Model and Linear Classfier; \textbf{FedFFT}: transfer the whole CLIP model (full fine-tuning). Our method (\textbf{\proj}) is highlighted in the green box. The figure is best viewed in color.
}

\label{fig:xxx}
\end{center}

% \vspace{-2.0em}

\end{figure*}

==> content/limit.tex <==
\section{Limitation}~\label{sec:limit}

While our proposed \proj framework demonstrates significant improvements in communication efficiency and model performance, there are several limitations and areas for future work that should be addressed.

\subsection{Scalability}

One of the primary limitations of our approach is the scalability of the framework. Although \proj reduces communication overhead by pruning less important layers, the approach still involves transferring significant amounts of data between clients and the server, particularly when the number of clients increases. To further enhance scalability, future research could explore more sophisticated data compression techniques or alternative methods for reducing the size of the model updates.


\subsection{Dynamic Rank of LoRA}

In our experiments, we used a fixed rank for the LoRA adapters. However, the optimal rank may vary across different layers and datasets. Allowing the rank to be dynamically adjusted based on the importance of each layer could further improve the efficiency and performance of the model. Future research could investigate adaptive mechanisms for dynamically determining the rank of LoRA adapters during training, possibly using reinforcement learning or other optimization techniques.








